PolyDiffuse: Polygonal Shape Reconstruction via Guided Set Diffusion Models

This paper presents PolyDiffuse, a novel structured reconstruction algorithm that transforms visual sensor data into polygonal shapes with Diffusion Models (DM), an emerging machinery amid exploding generative AI, while formulating reconstruction as a generation process conditioned on sensor data. The task of structured reconstruction poses two fundamental challenges to DM: 1) A structured geometry is a ``set'' (e.g., a set of polygons for a floorplan geometry), where a sample of $N$ elements has $N!$ different but equivalent representations, making the denoising highly ambiguous; and 2) A ``reconstruction'' task has a single solution, where an initial noise needs to be chosen carefully, while any initial noise works for a generation task. Our technical contribution is the introduction of a Guided Set Diffusion Model where 1) the forward diffusion process learns guidance networks to control noise injection so that one representation of a sample remains distinct from its other permutation variants, thus resolving denoising ambiguity; and 2) the reverse denoising process reconstructs polygonal shapes, initialized and directed by the guidance networks, as a conditional generation process subject to the sensor data. We have evaluated our approach for reconstructing two types of polygonal shapes: floorplan as a set of polygons and HD map for autonomous cars as a set of polylines. Through extensive experiments on standard benchmarks, we demonstrate that PolyDiffuse significantly advances the current state of the art and enables broader practical applications.

==> rebuttal/figure_hdmap_failure.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{pictures/rebuttal_failure_cases.pdf}
  \vspace{-1em}
   \caption{Failure examples of PolyDiffuse on the HD mapping task. We mark a predicted map element by \textcolor{red}{red} color if it is a true positive under both the Chamfer distance and the order-aware angle distance matching criteria. The thresholds used here are 1.0m and 10$^\circ$, respectively. See the text in the global response for discussions and analyses.
   }
   \vspace{-1em}
  \label{fig:floorplan_qualitative}
\end{figure}

==> rebuttal/table_floorplan_fps.tex <==
\begin{table}[th]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\vspace{-1.5em}
\caption{
The FPS of PolyDiffuse counts both the RoomFormer proposal generator and the GS-DM. The running time is measured with a single Nvidia RTX A5000 GPU. The same PolyDiffuse model is used as the Table.1 of the main paper.
}
\vspace{-0.8em}
\begin{tabular}{lccc@{\quad}cccccccccc}
\toprule
\multicolumn{4}{l}{Evaluation Level $\rightarrow$} &
\multicolumn{3}{c}{Room} & \multicolumn{3}{c}{Corner} & \multicolumn{3}{c}{Angle}\\
\cmidrule(r){5-7}	\cmidrule(r){8-10} \cmidrule(r){11-13}
Method & Stages & Steps & FPS  & Prec. & Rec. & F1 & Prec. & Rec. & F1 & Prec. & Rec. & F1 \\
\midrule
%
 RoomFormer & 1 & 1 & 29.9 & {96.3} & {96.2} & {96.2}  & {89.7} &  {86.7} &  {88.2} & 85.4 & 82.5 & {83.9} \\
 +\ourmethod & 2 & 2 & 11.7 & 96.9 & 96.4 & 96.6 & 90.3 & 87.1 & 88.7 & 85.8 & 82.8 & 84.3  \\
 +\ourmethod & 2 & 5 & 7.1 & 98.5 & 97.9 & 98.2 & 92.5 & 89.0 & 90.7 & 90.3 & 86.9 & 88.6 \\
+\ourmethod & 2 & 10 & 4.4 & \textbf{98.7} & \textbf{98.1} & \textbf{98.4}  & \textbf{92.8} &  \textbf{89.3} &  \textbf{91.0} & \textbf{90.8} & \textbf{87.4} & \textbf{89.1}  \\
\bottomrule
\end{tabular}
\label{tab:floorplan_fps}
\end{table}

==> rebuttal/table_hdmap_fps.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{
The FPS of PolyDiffuse counts both the MapTR proposal generator and the GS-DM. The running time in this table is measured on a single Nvidia RTX A5000 GPU. The PolyDiffuse here is retrained during rebuttal and has a slightly better performance than Table.2 of the main paper. 
}
\vspace{-0.8em}
\begin{tabular}{lccc@{\quad}cccccccc}
\toprule
\multicolumn{4}{l}{Matching Criterion $\rightarrow$} &
\multicolumn{4}{c}{Chamfer distance} & \multicolumn{4}{c}{+ Ordered angle distance} \\
\cmidrule(r){5-8}	\cmidrule(r){9-12}
Method &  Stages & Steps & FPS & AP$_{\textit{p}}$ & AP$_{\textit{d}}$ & AP$_{\textit{b}}$ & mAP & AP$_{\textit{p}}$ & AP$_{\textit{d}}$ & AP$_{\textit{b}}$ & mAP \\
\midrule
MapTR & 1 & 1 & 14.3 &  55.8 & \textbf{60.9} & 61.1 & 59.3 & 46.1 & 43.4 & 41.9 & 43.8 \\ 
+\ourmethod & 2 & 2 & 6.3 & 56.8 & 59.8 & 60.9 & 59.2 & 50.3 & 48.2 & 44.3 & 47.6 \\ 
+\ourmethod & 2 & 5 & 4.8 & 58.1 & 59.7 & 61.2 & 59.6 & 51.8 & 49.5 & 45.4 & 48.9 \\ 
+\ourmethod & 2 & 10 & 3.4 &  \textbf{58.2} & 59.7 & \textbf{61.3} & \textbf{59.7} & \textbf{52.0} & \textbf{49.5} & \textbf{45.4} & \textbf{49.0} \\ 
\bottomrule
\end{tabular}
\label{tab:hdmap_fps}
\end{table}

==> texts/algorithms/forward_training.tex <==
\algrenewcommand\algorithmicindent{0.5em}%
\begin{wrapfigure}{r}{0.5\textwidth}%
\begin{minipage}[t]{0.495\textwidth}
\begin{algorithm}[H]
  \caption{Training guidance network} \label{alg:training_guide}
  \small
  \begin{algorithmic}[1]
    \Repeat
      \State $\bx_0 \sim q(\bx_0)$
      \State $t \sim \mathrm{Uniform}(\{1, \dotsc, T\})$
      \State $\bepsilon\sim\mathcal{N}(\bzero,\bI)$
      \State Take gradient descent step on
      \Statex $\qquad \grad_\theta \left\| \bepsilon - \bepsilon_\theta(\sqrt{\bar\alpha_t} \bx_0 + \sqrt{1-\bar\alpha_t}\bepsilon, t) \right\|^2$
    \Until{converged}
  \end{algorithmic}
\end{algorithm}
\end{minipage}
\end{wrapfigure}

==> texts/tables/ablation_sampling_steps.tex <==
\begin{wraptable}{r}{0.5\linewidth}
% \vspace{-6mm}%
\caption{Results with different sampling steps and ODE solvers.}
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{ll@{\quad}ccc}
% \toprule
Solver & Steps & Room & Corner & Edge \\
\midrule
- & 1 & \\
%
DDIM & 2 (2) & \\ 
%
DDIM & 5 (5) & \\
%
DDIM & 10 (10) & \\
%
DDIM & 20 (20) & \\
%
Heun & 5 (9) & \\
%
Heun & 10 (19) & \\

\end{tabular}
\label{tab:ablation_steps}
\end{wraptable}

==> texts/tables/ablation_standard_dm.tex <==
% \begin{wraptable}{r}{0.5\linewidth}
% \vspace{-6mm}%
\begin{table}[]
\caption{The effect of the permutation-preserving diffusion. Results are reported in F1 score of three metric levels.}
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lc@{\quad}ccc}
% \toprule
Method & Steps & Room & Corner & Edge \\
\midrule
Base & 1 & 96.2 & 88.2 & 83.9 \\
\hdashline
%
\multirow{3}{*}{Standard} & 2 & 12.5 & 6.5 & 5.4 \\
%
 & 5 & 86.7 & 79.6 & 77.0\\ 
%
 & 10 & 90.4 & 83.6 & 81.1 \\ 
%
\hdashline
\multirow{3}{*}{GS-DM} & 2 & 
96.6 & 88.7 & 84.3 \\
%
 & 5 & 98.1 & 90.7 & 88.6 \\
%
 & 10 & 98.4 & 91.0 & 89.1 \\

\end{tabular}
\label{tab:ablation_dm}
\end{table}
% \end{wraptable}

==> texts/tables/ablation_training_schedule.tex <==
% \begin{wraptable}{r}{0.5\linewidth}
% \vspace{-6mm}%
\begin{table}[]
\caption{Performance of our method with different training schedule length}
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{ll@{\quad}ccc}
% \toprule
Method & Schedule & Room & Corner & Edge \\
\midrule
RoomFormer & $1\times$ & 96.2 & 88.2 & 83.9 \\
\hdashline
%
\multirow{4}{*}{PolyDiffuse} & $1\times$ & 98.3 & 90.6 & 88.6\\
& $1.5\times$ & 97.7 & 90.6 & 88.7  \\
%
 & $2\times$ &  \\ 
%
 & $2.5\times$ & 98.4 & 91.0 & 89.1 \\ 
 %
\end{tabular}
\label{tab:training_schedule}
\end{table}
% \end{wraptable}
